Resistive relativistic MHD simulations of astrophysical jets

Aims. The main goal of the present paper is to provide the first systematic numerical study of the propagation of astrophysical relativistic jets, in the context of high-resolution shock-capturing resistive relativistic magnetohydrodynamics (RRMHD) simulations. We aim at investigating different values and models for the plasma resistivity coefficient, and at assessing their impact on the level of turbulence, the formation of current sheets and reconnection plasmoids, the electromagnetic energy content, and the dissipated power. Methods. We use the PLUTO code for simulations and we assume an axisymmetric setup for jets, endowed with both poloidal and toroidal magnetic fields, and propagating in a uniform magnetized medium. The gas is assumed to be characterized by a realistic Synge-like equation of state (Taub equation), appropriate for such type of astrophysical jets. The Taub equation is combined here for the first time with the Implicit-Explicit Runge-Kutta time-stepping procedure, as required in RRMHD simulations. Results. The main result is that turbulence is clearly suppressed for the highest values of resistivity (low Lundquist numbers), current sheets are broader, and plasmoids are barely present, while for low values of resistivity results are very similar to ideal runs, where dissipation is purely numerical. We find that recipes employing a variable resistivity based on the advection of a jet tracer or on the assumption of a uniform Lundquist number improve on the use of a constant coefficient and are probably more realistic, preserving the development of turbulence and of sharp current sheets, possible sites for the acceleration of the non-thermal particles producing the observed high-energy emission.

==> referee_answer.tex <==
Dear Steve,

thank you very much for your prompt reply and your editorial decision of continuing the reviewing process.
Although the referee seems to have a conceptual problem with the resistive approach, we tried to address all the points raised in the report, even including some of them in the manuscript itself. 
We have submitted a revised version, where the debate on the role of the resistivity has been expanded. We hope that solves all the issues that the referee has with our approach.

Best regards,

Giancarlo Mattia and coauthors


-----------------------------------

Reply to the referee

We thank the referee for accepting to revise again our paper and for clarifying issues about the possible nature of microscopic particle acceleration, now reported in the Conclusions almost as stated in the referee's report.

We have removed a few lines from the Abstract and Introduction concerning particle acceleration, now it should be clear that the main goal of the paper is simply to assess for the first time the role of resistivity in the context of propagating astrophysical jets in the relativistic MHD regime. 
This is done quantitatively, contrary to what happens in simulations in the ideal case, where it is resolution and method dependent (see a new sentence in the Introduction).

Of course we still believe that our work and the resistive approach are important. The resistivity in macroscopic astrophysical sources is expected to be determined by unresolved turbulence rather than by collisions, so the effective Lunquist number could be still large, but much smaller. 
"Subgrid" processes like resistivity, dynamo etc. have been extensively adopted in the astrophysical community (not only in the context of astrophysical jets), providing a very good description of the "large-scale" impact of microscopic phenomena (see e.g. Liska et al 2020 on the dynamo-generated poloidal field in jet launching).
If the corresponding resistive electric field may have a role in accelerating particles is not commented in the paper, following the referee's suggestion. We have added some extra comments in the Conclusions.

As a final comment, with our work it is not our intention so say that all past and future ideal MHD simulations of jets are to be replaced by resistive ones, but is is important that the astrophysical community is aware of the role of physical resistivity over a purely numerical one (the latter being the only one present in ideal simulations): it may be much more 'realistic' a high resolution resistive run, than a low resolution ideal one. we hope the referee can agree on this point.

We believe that the current revision addresses all the points raised by the referee, thus being ready to be accepted for publication. 
We agree that the final word on the target audience (physicists or astrophysicists) should come from the Editor.

Best regards,

Giancarlo Mattia and coauthors
